Movies2Scenes: Using Movie Metadata to Learn Scene Representation

Understanding scenes in movies is crucial for a variety of applications such as video moderation, search, and recommendation. However, labeling individual scenes is a time-consuming process. In contrast, movie level metadata (e.g., genre, synopsis, etc.) regularly gets produced as part of the film production process, and is therefore significantly more commonly available. In this work, we propose a novel contrastive learning approach that uses movie metadata to learn a general-purpose scene representation. Specifically, we use movie metadata to define a measure of movie similarity, and use it during contrastive learning to limit our search for positive scene-pairs to only the movies that are considered similar to each other. Our learned scene representation consistently outperforms existing state-of-the-art methods on a diverse set of tasks evaluated using multiple benchmark datasets. Notably, our learned representation offers an average improvement of 7.9% on the seven classification tasks and 9.7% improvement on the two regression tasks in LVU dataset. Furthermore, using a newly collected movie dataset, we present comparative results of our scene representation on a set of video moderation tasks to demonstrate its generalizability on previously less explored tasks.

==> abstract_old.tex <==
\begin{abstract}

\vspace{-0.3cm}\noindent Labeling movie scenes is a time-consuming process which makes it difficult to apply end-to-end supervised methods for scene understanding. Moreover, directly using image based visual representations for scene understanding does not prove to be effective given the large domain gap between movies and standard image datasets. We address this challenge by proposing a novel contrastive learning approach that uses commonly available movie level metadata (\textit{e.g.}, co-watch, genre, synopsis) to learn a general purpose scene level representation. Our learned representation consistently outperforms existing state-of-the-art approaches on all of the \textbf{eleven tasks} evaluated using multiple benchmark datasets, with an average improvement of $7.9$\% on the seven classification tasks and $9.7$\% on the two regression tasks in the LVU dataset.
%We also demonstrate the effectiveness of our learned representation for video-moderation tasks evaluated using a newly collected large-scale internal movie dataset.
%To further demonstrate the generalizability of our learned representation, we present its comparative results on a set of video-moderation tasks evaluated using a newly collected large-scale movie dataset.
%To demonstrate the generalizability of our learned representation on previously less explored tasks, we present its comparative results on a set of video-moderation tasks evaluated using a newly collected large-scale movie dataset.
%Furthermore, we present comparative results of our representation on a set of video-moderation tasks evaluated using a newly collected large-scale movie dataset to demonstrate the effectiveness of our representation on previously less explored downstream tasks.
Furthermore, to demonstrate the generalizability and effectiveness of our representation on previously less explored downstream tasks, we present its comparative results on a set of video-moderation tasks evaluated using a newly collected large-scale movie dataset.

\end{abstract}

==> introduction_maxim.tex <==
\vspace{-0.5cm}
\section{Introduction}
\label{intro}

\noindent Learning general-purpose video representations is a subject of great interest to the computer vision community because these representations have far reaching applications in industry. Common applications are long-form video understanding, search, and recommendation. Notably, video representations can be used for video moderation where a classifier automatically assigns attributes (adult language, nudity, etc.) to long-form videos. The main challenge to learning on long-form videos is that labelled data is hard to come by. The length of long-form videos makes it laborious and expensive to label them. 

To learn in an environment of insufficient labelled data, the research community proposed multiple approaches~\cite{wang2020generalizing}. Contrastive learning~\cite{jaiswal2021survey} and pretext task learning~\cite{He_2020_CVPR}\cite{chen2020simple} emerged as promising directions. It's been demonstrated that contrastive learning on image-text pairs can achieve impressive results in zero-shot image classification~\cite{radford2021learning}. However, the representations learned from image-text pairs do not capture temporal, semantic, and thematic aspects of long-form video. Furthermore, it's impractical to extend image-text pairs to long-form video-text pairs because labeling long-form video with text is time consuming. As for representation learning that uses pretext tasks, it's unclear what kinds of pretext tasks are suitable for producing a general-purpose video representation. The previous pretext task approaches~\cite{He_2020_CVPR} have been shown to be less effective for long-form video understanding~\cite{Chen_2021_CVPR}. 

\begin{figure*}[!ht]
	%\teaser{
		\centering
		\includegraphics[width=1.0\textwidth]{teaser.jpg}
		\vspace{-0.6cm}\caption{\small {\textbf{Approach Overview -- } We employ commonly available movie-level information (\textit{e.g.}, co-watch, genre, synopsis) to define movie similarities which are used to learn scene-level representations. The figure illustrates a pair of similar movies where movie similarity is defined based on co-watch information, \textit{i.e.}, viewers who watched one movie often watched the second movie as well. Other movie-level data, \textit{e.g.}, genre and synopsis can be also used to define additional movie-level similarities. Our approach automatically selects thematically similar scenes from such similar movie-pairs and uses them in a contrastive learning setting to learn scene-level representations.}}\vspace{-0.5cm}
		\label{fig:teaser_fig}
		%}
\end{figure*}

In this paper, we propose a contrastive learning approach that uses video level metadata and the inherent narrative structure of the long-form video. Movies for example, have a natural hierarchical narrative structure that depicts a storyline. The storyline is presented through a sequence of scenes arranged in a particular order. Each scene, is in turn, a sequence of shots and each shot, is a sequence of frames captured from the same camera. Movies already come with a rich set of movie-level information, such as genre, synopsis, and co-watch statistics. Our intuition is that we can use movie-level information and the hierarchical structure of a movie storyline for representation learning. 

We posit that the most natural unit for movie representation learning are \textbf{scenes} because scenes are self-contained sections of a story. There's an added challenge to learning scene representations. Scenes have different number of shots that can last for dozens of minutes, which means any representation learning methodology has to be able to handle variable-length sequences of shots. To represent scenes as variable-length sequences of shots, we propose to use vision transformers~\cite{dosovitskiy2020vit} . 

Our \textbf{key contribution} is a contrastive learning framework for learning scene representations from movie-level information. We learn scene representations on an internal dataset $\mathsf{MovieCL30K}$ containing $30,340$ movies. We do this in two steps. First, we learn a movie-level similarity function using movie-level information. Second, we use movie similarity function to guide contrastive learning of scene representations (see Figure~\ref{fig:teaser_fig} for illustration). Our scene representations outperform state-of-the-art on \textbf{eleven downstream tasks} using multiple public benchmark datasets~\cite{Wu_2021_CVPR}\cite{huang2020movienet}\cite{rao2020local}. Our representations also outperform state-of-the-art on an internal movie moderation dataset $\mathsf{MCD}$. $\mathsf{MCD}$ is focused on large-scale video-moderation with $44,581$ video clips from $18,330$ movies and TV episodes containing $\mathsf{sex}$, $\mathsf{violence}$, and $\mathsf{drug}$-$\mathsf{use}$ activities.

The rest of this paper explains how we transfer movie level information down to scene level representations. In the ablation study, we show that it is the approach and not just the data that yields the new state-of-the-art results. 



